Efficient Federated Search for Retrieval-Augmented Generation using Lightweight Routing

Large language models (LLMs) achieve remarkable performance across domains but remain prone to hallucinations and inconsistencies. Retrieval-augmented generation (RAG) mitigates these issues by augmenting model inputs with relevant documents retrieved from external sources. In many real-world scenarios, relevant knowledge is fragmented across organizations or institutions, motivating the need for federated search mechanisms that can aggregate results from heterogeneous data sources without centralizing the data. We introduce RAGRoute, a lightweight routing mechanism for federated search in RAG systems that dynamically selects relevant data sources at query time using a neural classifier, avoiding indiscriminate querying. This selective routing reduces communication overhead and end-to-end latency while preserving retrieval quality, achieving up to 80.65% reductions in communication volume and 52.50% reductions in latency across three benchmarks, while matching the accuracy of querying all sources.

==> meta/cleverrefpatch.tex <==
% ---------- TEMPORARY PATCH for cleveref ≤ 0.21.6 ---------
\makeatletter
\AtBeginDocument{%
	% 1. Give \ltx@label its braces back
	\def\ltx@label#1{\cref@label{#1}}%
	
	% 2. Tell amsmath’s display-math helpers not to add braces
	\def\label@in@display@noarg#1{\cref@old@label@in@display{#1}}%
	
	% 3. Same again for the variant used while measuring multline
	\def\label@in@mmeasure@noarg#1{%
		\begingroup
		\measuring@false
		\cref@old@label@in@display{#1}%
		\endgroup
	}%
}
\makeatother
% ----------------------------------------------------------

==> plots/chart-matrix.tex <==
\input{plots/pgfplots-config.tex}
\noindent\begin{groupwidth}{3}
\begin{tikzpicture}
\pgfplotsset{cycle list/Set1-5}
\begin{groupplot}[
	width={150pt},
	group style = {
		group size = 3 by 3,
		horizontal sep=10mm,
		vertical sep=17mm,
	},
	colormap/Dark2,
	colormap/Paired,
	colormap/Set2,
	title style={at={(0.5,0.9)}},
	ymin=0%, ymax=100,
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
    %axis background/.style={fill=yellow!20},
	title={\mirage Communication Volume},
	ybar=0.5pt, bar width=5pt,
	ylabel={Communication volume},
	y unit={\mebi\byte},
	symbolic x coords={{all},{ragroute},{random}},
	xtick={{all},{ragroute},{random}},
	xticklabels={{all},\textbf{\sys},{random}},
	every axis plot/.append style={
        area legend,
        draw=black,
        line width=0.3pt,
        no markers,
    },
	cycle list name=bwcool9,
	enlarge x limits=0.15,
	x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

\addplot+[
    discard if not={strategy}{all},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{msg_size_sum_excl_train}/2^20},col sep=comma] 	{raw_data/ip_communication_MIRAGE.csv};

\addplot+[
    discard if not={strategy}{ragroute},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{msg_size_sum_excl_train}/2^20},col sep=comma] 	{raw_data/ip_communication_MIRAGE.csv};

\addplot+[
    discard if not={strategy}{random},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{msg_size_sum_excl_train}/2^20},col sep=comma] 	{raw_data/ip_communication_MIRAGE.csv};

\nextgroupplot[
    %axis background/.style={fill=yellow!20},
	title={\mirage Accuracy},
	ybar=0.5pt, bar width=5pt,
	ylabel={Accuracy},
	y unit={\%},
	symbolic x coords={{all},{ragroute},{random},{none}},
	xtick={{all},{ragroute},{random},{none}},
	xticklabels={{all},\textbf{\sys},{random},{none}},
	every axis plot/.append style={
        area legend,
        draw=black,
        line width=0.3pt,
        no markers,
    },
	cycle list name=bwcool9,
	enlarge x limits=0.15,
	x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
    ymin=55
]

%\addplot+[
%]
%table[	col sep=comma, x={SUFFIX}, y expr={100*\thisrow{MEAN}},
%]
%{raw_data/mid_accuracy_MIRAGE.csv};

\addplot+[
    discard if not={strategy}{all},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{avg_correct}*100},col sep=comma] 	{raw_data/ip_accuracy_MIRAGE.csv};

\addplot+[
    discard if not={strategy}{ragroute},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{avg_correct}*100},col sep=comma] 	{raw_data/ip_accuracy_MIRAGE.csv};

\addplot+[
    discard if not={strategy}{random},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{avg_correct}*100},col sep=comma] 	{raw_data/ip_accuracy_MIRAGE.csv};

\addplot+[
    discard if not={strategy}{none},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{avg_correct}*100},col sep=comma] 	{raw_data/ip_accuracy_MIRAGE.csv};


\nextgroupplot[
    %axis background/.style={fill=yellow!20},
    ybar stacked,
	title={\mirage time breakdown},
    bar width=5pt,
	legend columns=2,
	legend style={fill=none, at={(0.5,1.2)}},
	ylabel={Time},
	y unit={s},
	symbolic x coords={{all},{ragroute},{random},{none}},
    xticklabels={{all},\textbf{\sys},{random},{none}},
    xtick={{all},{ragroute},{random},{none}},
	every axis plot/.append style={
        area legend,
        draw=black,
        line width=0.3pt,
        no markers,
    },
    cycle list name=bwcool9,
    cycle list shift=4,
	enlarge x limits=0.15,
	x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

\foreach \qa in {{SELECTION_TIME},{EMBEDDING_TIME}, {DOC_SELECT_TIME},{RERANK_TIME},{GENERATE_TIME}}{
	\addplot+[
	]
	table[	col sep=comma, x={SUFFIX}, y={MEAN},
	discard if not={STRATEGY}{\qa},
	]
	{raw_data/ip_times_MIRAGE.csv};
}

\legend{{source select},{embed},{doc select},{rerank},{generate}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
    %axis background/.style={fill=yellow!20},
    title={\mmlu Communication Volume},
    ybar=0.5pt, bar width=5pt,
    ylabel={Communication volume},
    y unit={\mebi\byte},
    symbolic x coords={{all},{ragroute},{random}},
    xtick={{all},{ragroute},{random}},
    xticklabels={{all},\textbf{\sys},{random}},
    every axis plot/.append style={
        area legend,
        draw=black,
        line width=0.3pt,
        no markers,
    },
    cycle list name=bwcool9,
    enlarge x limits=0.15,
   	x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

\addplot+[
    discard if not={strategy}{all},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{msg_size_sum_excl_train}/2^20},col sep=comma] 	{raw_data/ip_communication_mmlu.csv};

\addplot+[
    discard if not={strategy}{ragroute},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{msg_size_sum_excl_train}/2^20},col sep=comma] 	{raw_data/ip_communication_mmlu.csv};

\addplot+[
    discard if not={strategy}{random},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{msg_size_sum_excl_train}/2^20},col sep=comma] 	{raw_data/ip_communication_mmlu.csv};


\nextgroupplot[
    %axis background/.style={fill=yellow!20},
    title={\mmlu Accuracy},
    ybar=0.5pt, bar width=5pt,
    ylabel={Accuracy},
    y unit={\%},
    symbolic x coords={{all},{ragroute},{random},{none}},
    xtick={{all},{ragroute},{random},{none}},
    xticklabels={{all},\textbf{\sys},{random},{none}},
    every axis plot/.append style={
        area legend,
        draw=black,
        line width=0.3pt,
        no markers,
    },
    cycle list name=bwcool9,
    enlarge x limits=0.15,
    ymin=60,
    x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

%\addplot+[
%    ]
%table[	col sep=comma, x={SUFFIX}, y expr={100*\thisrow{MEAN}},
%    ]
%{raw_data/mid_accuracy_MMLU.csv};

\addplot+[
    discard if not={strategy}{all},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{avg_correct}*100},col sep=comma] 	{raw_data/ip_accuracy_MMLU.csv};

\addplot+[
    discard if not={strategy}{ragroute},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{avg_correct}*100},col sep=comma] 	{raw_data/ip_accuracy_MMLU.csv};

\addplot+[
    discard if not={strategy}{random},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{avg_correct}*100},col sep=comma] 	{raw_data/ip_accuracy_MMLU.csv};

\addplot+[
    discard if not={strategy}{none},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{avg_correct}*100},col sep=comma] 	{raw_data/ip_accuracy_MMLU.csv};


\nextgroupplot[
    %axis background/.style={fill=yellow!20},
    ybar stacked,
    title={\mmlu time breakdown},
    bar width=5pt,
    legend columns=-1,
    legend style={fill=none, at={(0.5,1.2)}},
    ylabel={Time},
    y unit={s},
    symbolic x coords={{all},{ragroute},{random},{none}},
    xticklabels={{all},\textbf{\sys},{random},{none}},
    xtick={{all},{ragroute},{random},{none}},
    every axis plot/.append style={
        area legend,
        draw=black,
        line width=0.3pt,
        no markers,
    },
    cycle list name=bwcool9,
    cycle list shift=4,
    enlarge x limits=0.15,
     x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

\foreach \qa in {{SELECTION_TIME},{EMBEDDING_TIME},{DOC_SELECT_TIME},{RERANK_TIME},{GENERATE_TIME}}{
    \addplot+[
    ]
    table[	col sep=comma, x={SUFFIX}, y expr={\thisrow{MEAN}},
    discard if not={STRATEGY}{\qa},
    ]
    {raw_data/ip_times_MMLU.csv};
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
    xshift={75pt},
    %axis background/.style={fill=yellow!20},
    title={\febrag Communication Volume},
    ybar=0.5pt, bar width=5pt,
    ylabel={Communication volume},
    y unit={\mebi\byte},
    symbolic x coords={{all},{ragroute},{random}},
    xtick={{all},{ragroute},{random}},
    xticklabels={{all},\textbf{\sys},{random}},
    every axis plot/.append style={
        area legend,
        draw=black,
        line width=0.3pt,
        no markers,
    },
    cycle list name=bwcool9,
    enlarge x limits=0.15,
    x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

\addplot+[
    discard if not={strategy}{all},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{msg_size_sum_excl_train}/2^20},col sep=comma] 	{raw_data/ip_communication_FeB4RAG.csv};

\addplot+[
    discard if not={strategy}{ragroute},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{msg_size_sum_excl_train}/2^20},col sep=comma] 	{raw_data/ip_communication_FeB4RAG.csv};

\addplot+[
    discard if not={strategy}{random},
	bar shift=-0.1pt,
]
table[x={strategy},y expr={\thisrow{msg_size_sum_excl_train}/2^20},col sep=comma] 	{raw_data/ip_communication_FeB4RAG.csv};


\nextgroupplot[
    xshift={75pt},
    %axis background/.style={fill=yellow!20},
    ybar stacked,
    title={\febrag time breakdown},
    bar width=5pt,
    legend columns=-1,
    legend style={fill=none, at={(0.5,1.2)}},
    ylabel={Time},
    y unit={s},
    symbolic x coords={{all},{ragroute},{random}},
    xticklabels={{all},\textbf{\sys},{random}},
    xtick={{all},{ragroute},{random}},
    every axis plot/.append style={
        area legend,
        draw=black,
        line width=0.3pt,
        no markers,
    },
    cycle list name=bwcool9,
    cycle list shift=4,
    enlarge x limits=0.15,    
    x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

\foreach \qa in {{SELECTION_TIME},{EMBEDDING_TIME},{DOC_SELECT_TIME},{RERANK_TIME},{GENERATE_TIME}}{
    \addplot+[
    ]
    table[	col sep=comma, x={SUFFIX}, y expr={\thisrow{MEAN}},
    discard if not={STRATEGY}{\qa},
    ]
    {raw_data/ip_times_feb4rag.csv};
}


\end{groupplot}

%\node[text width=96pt, align=center] at (0.75,-3.7) {\color{black} Bar labels indicate the normalized comm. cost w.r.t. \ofl};
%\node at (1.9,-1) {\emph{(a)}};
%\node at (8.9,-1) {\emph{(b)}};
%\node at (12.1,-1) {\emph{(c)}};

\end{tikzpicture}
\end{groupwidth}

==> plots/communication.tex <==
\input{plots/pgfplots-config.tex}
\noindent%\begin{groupwidth}{3}
\begin{tikzpicture}
\pgfplotsset{cycle list/Set1-5}
\begin{groupplot}[
	%height={3.4cm},
	group style = {
		group size = 3 by 1,
		horizontal sep=8mm,
		vertical sep=17mm,
	},
	colormap/Dark2,
	colormap/Paired,
	colormap/Set2,
	title style={at={(0.5,0.9)}},
	ymin=0
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
    width={100pt},
	%xshift={7mm},
	title={\febrag},
	%width={125.8pt},
	ybar=0.5, bar width=4.5pt,
	legend columns=-1,
	legend style={fill=none, at={(1.1,1.15)}},
	%xlabel={Question set},
	xlabel style={at={(1,-0.5)}},
	ylabel={Data sources},
	ylabel style={at={(-0.2,0.5)}},
	%y unit={\%},
	symbolic x coords={{all},{ragroute},{random}},
	xtick={{all},{ragroute},{random}},
	xticklabels={{all},{\textbf{\sys}},{random}},
	%ymin=0,
	%yticklabels={\empty},
	every axis plot/.append style={fill,draw=none,no markers},
	cycle list name=bwcool9,
	enlarge x limits=0.15,
	x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

%	\addplot+[
%	]
%	table[	col sep=comma, x={SUFFIX}, y expr={\thisrow{TOTAL}/10^3},
%	]
%	{raw_data/mid_queries_FeB4RAG.csv};

 \addplot+[
	discard if not={strategy}{all},
	bar shift=-0.1pt,
]
table[x={strategy},y={avg_num_data_sources},col sep=comma] {raw_data/ip_queries_feb4rag.csv};

 \addplot+[
	discard if not={strategy}{ragroute},
	bar shift=-0.1pt,
]
table[x={strategy},y={avg_num_data_sources},col sep=comma] {raw_data/ip_queries_feb4rag.csv};

 \addplot+[
	discard if not={strategy}{random},
	bar shift=-0.1pt,
]
table[x={strategy},y={avg_num_data_sources},col sep=comma] {raw_data/ip_queries_feb4rag.csv};

%\legend{{Naive},{Relevant},{Predicted}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nextgroupplot[
	width={100pt},
	%xshift={10mm},
	title={\mirage},
	%width={125.8pt},
	ybar=0.5pt, bar width=4.5pt,
	legend columns=-1,
	legend style={fill=none,at={(0.25,1.2)}},
	symbolic x coords={{all},{ragroute},{random}},
	xtick={{all},{ragroute},{random}},
	xticklabels={{all},{\textbf{\sys}},{random}},
	%ymin=0,
	%yticklabels={\empty},
	every axis plot/.append style={fill,draw=none,no markers},
	cycle list name=bwcool9,
	enlarge x limits=0.12,
	x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

\addplot+[
	discard if not={strategy}{all},
	bar shift=-0.1pt,
]
table[x={strategy},y={avg_num_data_sources},col sep=comma] 	{raw_data/ip_queries_MIRAGE.csv};

\addplot+[
	discard if not={strategy}{ragroute},
	bar shift=-0.1pt,
]
table[x={strategy},y={avg_num_data_sources},col sep=comma] 	{raw_data/ip_queries_MIRAGE.csv};

\addplot+[
	discard if not={strategy}{random},
	bar shift=-0.1pt,
]
table[x={strategy},y={avg_num_data_sources},col sep=comma] 	{raw_data/ip_queries_MIRAGE.csv};


%\legend{{Naive},{Relevant},{Predicted by \textbf{\sys}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nextgroupplot[
    width={100pt},
    %xshift={10mm},
    title={\mmlu},
    %width={125.8pt},
    ybar=0.5pt, bar width=4.5pt,
    legend columns=-1,
    legend style={fill=none,at={(0.25,1.2)}},
    symbolic x coords={{all},{ragroute},{random}},
    xtick={{all},{ragroute},{random}},
    xticklabels={{all},{\textbf{\sys}},{random}},
    %ymin=0,
    %yticklabels={\empty},
    every axis plot/.append style={fill,draw=none,no markers},
    cycle list name=bwcool9,
    enlarge x limits=0.12,
    x tick label style={rotate=30,anchor=east,yshift=-2mm,xshift=0.5mm},
]

\addplot+[
	discard if not={strategy}{all},
	bar shift=-0.1pt,
]
table[x={strategy},y={avg_num_data_sources},col sep=comma] 	{raw_data/ip_queries_MMLU.csv};

\addplot+[
	discard if not={strategy}{ragroute},
	bar shift=-0.1pt,
]
table[x={strategy},y={avg_num_data_sources},col sep=comma] 	{raw_data/ip_queries_MMLU.csv};

\addplot+[
	discard if not={strategy}{random},
	bar shift=-0.1pt,
]
table[x={strategy},y={avg_num_data_sources},col sep=comma] 	{raw_data/ip_queries_MMLU.csv};

%\legend{{Naive},{Relevant},{Predicted by \textbf{\sys}}}

\end{groupplot}

%\node[text width=96pt, align=center] at (0.75,-3.7) {\color{black} Bar labels indicate the normalized comm. cost w.r.t. \ofl};
%\node at (1.9,-1) {\emph{(a)}};
%\node at (8.9,-1) {\emph{(b)}};
%\node at (12.1,-1) {\emph{(c)}};

\end{tikzpicture}
%\end{groupwidth}

==> plots/pgfplots-config.tex <==
\pgfplotsset{compat=newest,
    width=\linewidth, height=3.5cm,
    every axis/.append style={
     semithick,
     ymajorgrids=true,
    },
    legend style={
     draw=none,
     fill=white,
     anchor=south,
     at={(0.5, 1)},
     font=\small,
    },
	{cycle list/Set1},
    cycle list name=Set1,
    cycle multiindex* list={
    	Set1\nextlist
    	{dashed,solid,dotted,dashdotted,densely dashdotdotted}\nextlist
    	mark list*\nextlist
    },
    legend cell align=left,
    xtick align=outside,
    xtick pos=bottom,
    major tick length=1mm,
    /pgfplots/short line legend/.style={
     legend image code/.code={
         \draw[mark repeat=2,mark phase=2,##1]
             plot coordinates {
                 (0cm,0cm)
                     (0.2cm,0cm)
                     (0.4cm,0cm)
             };%
     }
    },
    /pgfplots/ybar legend/.style={
    /pgfplots/legend image code/.code={%
         \draw[##1,/tikz/.cd,yshift=-0.25em]
             (0cm,0cm) rectangle (4pt,6pt);},
    },
    /pgfplots/xbar legend/.style={
    /pgfplots/legend image code/.code={%
         \draw[##1,/tikz/.cd,yshift=-0.25em]
             (0cm,0cm) rectangle (4pt,6pt);},
    },
    unit code/.code={\si{#1}},
    tick label style = {font=\sansmath\sffamily},
    every axis label = {font=\sffamily},
    legend style = {font=\sffamily},
    label style = {font=\sffamily},
    select coords between index/.style 2 args={
    	x filter/.code={
    		\ifnum\coordindex<#1\def\pgfmathresult{}\fi
    		\ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }},
	discard if not/.style 2 args={
		x filter/.code={
			\edef\tempa{\thisrow{#1}}
			\edef\tempb{#2}
			\ifx\tempa\tempb
			\else
			\def\pgfmathresult{inf}
			\fi
	}},
	discard if/.style 2 args={
	x filter/.code={%
		\edef\tempa{\thisrow{#1}}%
		\edef\tempb{#2}%
		\ifx\tempa\tempb
		\def\pgfmathresult{nan}%
		\fi
	}},
}




==> plots/routing.tex <==
\input{plots/pgfplots-config.tex}
\noindent%\begin{groupwidth}{1}
\begin{tikzpicture}
\pgfplotsset{cycle list/Set1-5}
\begin{groupplot}[
	width={258pt}, 
	%height={3.4cm},
	group style = {
		group size = 1 by 1,
		horizontal sep=2mm,
		vertical sep=17mm,
	},
	colormap/Dark2,
	colormap/Paired,
	colormap/Set2,
	title style={at={(0.5,0.9)}},
	ymin=0
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nextgroupplot[
	title={Top 32},
	ybar=0.5pt, bar width=5pt, 
	enlarge x limits=0.3,
	legend style={at={(0.55,1.05)}},
	legend columns=-1,
	ylabel={Relevance score},
	y unit={\%},
	xlabel={Corpus},
	symbolic x coords={{pubmed},{statpearls},{wikipedia},{textbooks}},
	xtick=data,
	%ymin=0, 
	%yticklabels={\empty},
	every axis plot/.append style={fill,draw=none,no markers},
	cycle list name=Set2,
	enlarge x limits=0.15,
]

% \foreach \qa in {pubmedqa,medqa,bioasq,medmcqa,mmlu-med}{
% 	\addplot+[%bar shift=-3.5pt, 
% 	%postaction={pattern=north west lines, pattern color=gray}, 
% 	%error bars/.cd, error bar style={black}
% 	]
% 	table[	col sep=comma, x={Corpus}, y={\qa}, 
% 	%y error expr={1.96*\thisrow{acc_std}/sqrt(3)},
% 	%select coords between index={0}{2}
% 	]
% 	{raw_data/ip_querying_distribution_top_15.csv};
% 	%\addlegendentry{\qa}
% }

\addplot+[
    postaction={pattern=north east lines, pattern color=black}
]
table[col sep=comma, x={Corpus}, y={pubmedqa}]
{raw_data/ip_querying_distribution_top_15.csv};

\addplot+[
    postaction={pattern=north west lines, pattern color=black}
]
table[col sep=comma, x={Corpus}, y={medqa}]
{raw_data/ip_querying_distribution_top_15.csv};

\addplot+[
    postaction={pattern=horizontal lines, pattern color=black}
]
table[col sep=comma, x={Corpus}, y={bioasq}]
{raw_data/ip_querying_distribution_top_15.csv};

\addplot+[
    postaction={pattern=vertical lines, pattern color=black}
]
table[col sep=comma, x={Corpus}, y={medmcqa}]
{raw_data/ip_querying_distribution_top_15.csv};

\addplot+[
    postaction={pattern=dots, pattern color=black}
]
table[col sep=comma, x={Corpus}, y={mmlu-med}]
{raw_data/ip_querying_distribution_top_15.csv};


\legend{pubmedqa,medqa,bioasq,medmcqa,mmlu-med}

\end{groupplot}

%\node[text width=96pt, align=center] at (0.75,-3.7) {\color{black} Bar labels indicate the normalized comm. cost w.r.t. \ofl};
%\node at (1.9,-1) {\emph{(a)}};
%\node at (8.9,-1) {\emph{(b)}};
\node at (0.15,2.3) {Question set:};

\end{tikzpicture}
%\end{groupwidth}

==> sections/abstract.tex <==
\begin{abstract}

Large language models (LLMs) have demonstrated remarkable performance across various domains but remain susceptible to hallucinations and inconsistencies, limiting their reliability.
Retrieval-augmented generation (RAG) addresses these limitations by enriching the LLM input with relevant documents retrieved from external sources.
Existing RAG workflows typically leverage a single data source.
In many real-world scenarios, however, relevant knowledge is fragmented across organizations or institutions, making it essential to collaboratively leverage these diverse and distributed sources of information.
To this end, we introduce \textsc{RAGRoute}, a novel mechanism for federated RAG search across multiple heterogeneous data sources.
\textsc{RAGRoute} dynamically selects relevant data sources at query time using a lightweight neural network classifier, eliminating the need to query all sources indiscriminately.
This selective routing significantly improves retrieval efficiency by lowering communication overhead and reducing end-to-end latency.
We evaluate \textsc{RAGRoute} using three benchmarks, \textsc{MIRAGE}, \textsc{MMLU} and \textsc{FeB4RAG}.
Our experiments show that \textsc{RAGRoute} reduces the retrieval communication volume by up to 80.65\% and end-to-end latency by up to 52.50\%, while maintaining high retrieval quality and matching the end-to-end accuracy of querying all sources.


\end{abstract}


==> sections/system_architecture.tex <==
\section{System architecture and implementation}
\label{sec:architecture}
We implement \sys and now describe our system architecture which is visualized in~\Cref{fig:architecture}.

\subsection{System architecture}
\sys consists of the following components and each one is implemented as a separate process.

\textbf{Coordinator and HTTP server.}
At the core of \sys is a main process containing a coordinator and a HTTP server.
The HTTP server receives incoming web requests from users and returns responses once the query is processed by \sys.
When receiving such a request, the query inside the request is forwarded to the coordinator which manages communication between various other components.

\textbf{Router.}
The coordinator first forwards the query to the routing process (step 3 in~\Cref{fig:architecture}).
This routing process has the relevant embedding models loaded in memory and also hosts the \sys router model.
After embedding generation, these embeddings are forwarded to the \sys router model (step 4), which outputs a list of relevant data sources.
The identifiers of these data sources and the generated embeddings are returned to the coordinator (step 5).

\textbf{Data sources.}
Next, the coordinator sends the compatible embedding to each of the relevant data sources \emph{in parallel}.
Based on this embedding, these data sources retrieve the top-$k_{retrieve}$ relevant documents and return these documents to the coordinator.
After the coordinator receives a reply from all data sources it reranks and filters the documents, resulting in a top-$k$ list of relevant document chunks.
In our implementation, each data source is implemented as a separate process.
In deployed settings, these data sources might be hosted on the same machine or be distributed across multiple machines.

\textbf{\ac{LLM} engine.}
Finally, the coordinator constructs the prompt that will be forwarded to the \ac{LLM} engine.
This prompt contains the query, originally sent by the user, and the retrieved documents.
Since the length of the concatenated chunks and query might exceed the context size of the \ac{LLM}, the coordinator first tokenizes all chunks and truncates the tokenized data to avoid this.
The prompt is then forwarded to the \ac{LLM} engine which runs as a separate process.
The \ac{LLM} returns its response to the coordinator (step 9) and a reply is returned to the user (step 10 and 11).


\subsection{Implementation details}
We implement the system architecture in \Cref{fig:architecture} in the Python programming language.
Our implementation is open source and available on GitHub.\footnote{https://anonymous.4open.science/r/ragroute/README.md.}
Our implementation adopts an event-driven programming model with the \texttt{asyncio} library.
We also use the \textsc{ZeroMQ} library for messaging between the different subprocesses and \textsc{AIOHTTP} for the HTTP server.
We use the \textsc{Ollama} framework for inference which runs as a separate process and provides a convenient way to load and run inference with different \acp{LLM}~\cite{ollama}.
For the embedding models, we use the \textsc{PyTorch} library.
